Equivariant $Q$ Learning in Spatial Action Spaces

Recently, a variety of new equivariant neural network model architectures have been proposed that generalize better over rotational and reflectional symmetries than standard models. These models are relevant to robotics because many robotics problems can be expressed in a rotationally symmetric way. This paper focuses on equivariance over a visual state space and a spatial action space -- the setting where the robot action space includes a subset of $\rm{SE}(2)$. In this situation, we know a priori that rotations and translations in the state image should result in the same rotations and translations in the spatial action dimensions of the optimal policy. Therefore, we can use equivariant model architectures to make $Q$ learning more sample efficient. This paper identifies when the optimal $Q$ function is equivariant and proposes $Q$ network architectures for this setting. We show experimentally that this approach outperforms standard methods in a set of challenging manipulation problems.

==> dian_working.tex <==
\subsubsection{Only Using Equivariant Network in $q_1$ or $q_2$}
\begin{figure}[H]
\centering
\subfloat[House Building]{\includegraphics[width=0.25\linewidth]{image/exp/asr/h4_q1q2.png}}
\subfloat[Box Palletizing 12]{\includegraphics[width=0.25\linewidth]{image/exp/asr/box12_q1q2.png}}
\subfloat[Box Palletizing 18]{\includegraphics[width=0.25\linewidth]{image/exp/asr/box18_q1q2.png}}
\subfloat[Bin Packing]{\includegraphics[width=0.25\linewidth]{image/exp/asr/bbp_q1q2.png}}
\caption{Comparison of four variations of equivariant/conventional and $q_1$/$q_2$ combinations}
\label{fig:exp_asr_q1q2}
\end{figure}

In this ablation study, we evaluate the effect of the equivariant network by only applying it in $q_1$ or $q_2$. There are four variations: 1) Equivariant $q_1$ + Equivariant $q_2$: both $q_1$ and $q_2$ use the equivariant network; 2) Equivariant $q_1$ + Conventional $q_2$: $q_1$ uses the equivariant network, $q_2$ uses the conventional convolutional network; 3) Conventional $q_1$ + Equivariant $q_2$: $q_1$ uses the conventional convolutional network, $q_2$ uses the equivariant network; 4) Conventional $q_1$ + Conventional $q_2$: both $q_1$ and $q_2$ use conventional convolutional network. The results are shown in Figure~\ref{fig:exp_asr_q1q2}, where Using the equivariant network in both $q_1$ and $q_2$ (blue) always shows the best performance. Note that applying the equivariant network in $q_2$ (red) generally demonstrates a greater improvement. This is because $q_2$ is responsible for providing the TD target.
